PointContrast: Unsupervised Pre-training for 3D Point Cloud Understanding

Arguably one of the top success stories of deep learning is transfer learning. The finding that pre-training a network on a rich source set (eg., ImageNet) can help boost performance once fine-tuned on a usually much smaller target set, has been instrumental to many applications in language and vision. Yet, very little is known about its usefulness in 3D point cloud understanding. We see this as an opportunity considering the effort required for annotating data in 3D. In this work, we aim at facilitating research on 3D representation learning. Different from previous works, we focus on high-level scene understanding tasks. To this end, we select a suite of diverse datasets and tasks to measure the effect of unsupervised pre-training on a large source set of 3D scenes. Our findings are extremely encouraging: using a unified triplet of architecture, source dataset, and contrastive loss for pre-training, we achieve improvement over recent best results in segmentation and detection across 6 different benchmarks for indoor and outdoor, real and synthetic datasets -- demonstrating that the learned representation can generalize across domains. Furthermore, the improvement was similar to supervised pre-training, suggesting that future efforts should favor scaling data collection over more detailed annotation. We hope these findings will encourage more research on unsupervised pretext task design for 3D deep learning.

==> tex/dataset.tex <==
In what follows we measure the transferability of the descriptors learned at pre-training. To make a comprehensive evaluation, we utilize multiple datasets and benchmarks. This allows us to cover, on the datasets side, both indoor and outdoor complex scenes as well as individual synthetic objects. These also exhibit variability in sensor type, reconstruction algorithms, etc. Table~\ref{tab:dataset_summary} summarizes the main attributes of the different datasets. On the task side, we go beyond low-level tasks previously tested in other works like registration or pose estimation, and cover higher level scene understanding, namely  semantic segmentation and object detection. Next, we describe the different datasets. The associated tasks are described in the results section. 

% \input{tex/tables/dataset_summary}

\paragraph{S3DIS \CITE}
dataset comprises 3D scans of 6 large-scale indoor areas collected from 3 office buildings. The scans are represented as pointclouds and annotated semantic labels of 13 object categories. Among the datasets utilized here S3DIS is probably the most similar to ScanNet, with the main difference being the content of the the scenes which is mostly offices as opposed to the more diverse room types in ScanNet. 

\paragraph{SUN RGB-D \CITE}
is a collection of single view RGB-D captures curated from 3 sources: NYU depth v2~\cite{silberman2012indoor}, Berkeley B3DO~\cite{janoch2013category}, and SUN3D~\cite{xiao2013sun3d}. The train set contains 5K images annotated with amodal, 3D oriented bounding boxes for objects from 37 categories. Camera parameters are provided, enabling the conversion of depth channels to pointclouds in world coordinates. Presenting high diversity in the (real) room content, the main difference between SUN RGB-D and ScanNet is that the former is single-view. 

\paragraph{ShapeNet \cite{shapenet2015}}
is a large-scale dataset of synthetic 3D shapes of 16 common categories. Is was curated by collecting CAD models from online open-sourced 3D repositories. Here we utilize ShapeNet part \cite{Yi16} which further added part annotations to ShapeNet models segmenting them into 2-5 parts. We follow many previous works (e.g. \cite{qi2017pointnet}) and uniformly sample pointclouds of size 1024 from each model. Albeit containing overlapping indoor object categories with ScanNet, this dataset in substantially different as it is synthetic, and contains objects in isolation lacking the scene context. 

\paragraph{Synthia \cite{ros2016synthia}}
is a large synthetic dataset designed to facilitate the training of deep neural networks for visual inference in driving scenarios. Photo-realistic renderings are generated from a virtual city, allowing dense and precise annotations of 13 semantic classes, together with pixel-accurate depth. We follow the train/val/test split as prescribed by \cite{choy20194d} in the clean setting. In the context of this work, Synthia is especially interesting since it is probably the most distant from ScanNet. Ergo, transferability to Synthia would imply that the pretext task was able to extract \textit{universal} features that can adapt to other domains.    

==> tex/tables/segmentation_supervised_pretraining.tex <==
\begin{table*}[t!]
\centering
\tablestyle{1.2pt}{1.1}
\begin{tabular}{l | c c}
methods & mIoU & mAcc \\
\hshline
Training from scratch & 68.2 & 75.5 \\
\hline
Supervised Pretraining & \textbf{71.2}  & \textbf{77.8} \\
Unsupervised PointContrast & \textbf{70.9} & \textbf{77.0} \\
\end{tabular}
\caption{\textbf{Stanford Area 5 Test (Fold 1) (S3DIS).} 
}
\label{tab:S3DIS:supervised}
\end{table*}

